Games Without Frontiers: Investigating Video Games as a Covert Channel

The Internet has become a critical communication infrastructure for citizens to organize protests and express dissatisfaction with their governments. This fact has not gone unnoticed, with governments clamping down on this medium via censorship, and circumvention researchers working to stay one step ahead. In this paper, we explore a promising new avenue for covert channels: real-time strategy-video games. Video games have two key features that make them attractive cover protocols for censorship circumvention. First, due to the popularity of gaming platforms such as Steam, there are a lot of different video games, each with their own protocols and server infrastructure. Users of video-game-based censorship-circumvention tools can therefore diversify across many games, making it difficult for the censor to respond by simply blocking a single cover protocol. Second, games in the same genre have many common features and concepts. As a result, the same covert channel framework can be easily adapted to work with many different games. This means that circumvention tool developers can stay ahead of the censor by creating a diverse set of tools and by quickly adapting to blockades created by the censor. We demonstrate the feasibility of this approach by implementing our coding scheme over two real-time strategy-games (including a very popular closed-source game). We evaluate the security of our system prototype -- Castle -- by quantifying its resilience to a censor-adversary, its similarity to real game traffic, and its ability to avoid common pitfalls in covert channel design. We use our prototype to demonstrate that our approach can provide throughput which is amenable to transfer of textual data, such at e-mail, SMS messages, and tweets, which are commonly used to organize political actions.

==> background.tex <==
%\section{Background}\label{sec:background}

%I implemented this re org...  \Pnote{The contents of this section are really
%random. I would advocate moving 2.2 to 3 and leaving arms race and threat
%model here, or even making them each their own sections}

\section{Background}\label{subsec:arms-race}

Censorship circumvention tools face an arms race as they work to evade
increasingly powerful and motivated censors. Tools which have distinctive 
features are detected and blocked by censors (\eg Tor is actively targeted 
by censors around the world~\cite{tor-blocked}). As a result, there is 
increasing interest in disguising censorship circumvention traffic as benign 
protocols. SkypeMorph~\cite{skypemorph} and StegoTorus~\cite{stegotorus} are 
two pluggable transports~\cite{tor-pt} for Tor which aim to mask Tor traffic 
as Skype traffic, and a combination of Skype, HTTP and Ventrilo, respectively. 

While these pluggable transports are able to capture features of the traffic
they aim to imitate (\eg inter-packet timings, packet size distributions),
Houmansadr \etal \cite{parrot-is-dead} point out that imitating a protocol is
not enough to evade detection -- i.e., if circumvention endpoints do not run
the application they aim to hide within, they are vulnerable to censors who may
perform active probing to observe that the endpoint does not actually implement
the full functionality of the mimicked application. As such, Houmansadr \etal
advocate that circumvention schemes should actually run the application they
are using as cover, rather than mimicking properties of the cover traffic.

Towards this goal, FreeWave uses the Skype application as a modem to
transmit IP data between two endpoints~\cite{freewave}. However,
Geddes \etal demonstrate that even running the cover application is
not enough to avoid detection by censors~\cite{cover-your-acks} --
i.e., approaches like FreeWave may be detected via discrepancies
between the application's regular behavior and its behavior when being
used as a covert channel.  They classify these discrepancies into
three categories: (1) architectural mismatches between communication
patterns of the application when it is acting as a covert channel \vs
regular operation, (2) channel mismatches between reliability
requirements of the application and the covert traffic and (3) content
mismatches where the packet contents of the application differ because
of the covert traffic being sent in place of regular application
traffic.

Thus, circumventors are in a race to design new covert channels that are
difficult to detect, while censors search for low-cost mechanisms to
distinguish legitimate traffic from covert channels. 

In this paper, we argue that multi-player games as a covert channel
presents a solution that can tip the scales heavily in the favor of
circumvention tool developers.  The large number of games and common
features of games within a given genre facilitate quick adaptation of
existing game-based covert channels to new games.

The number of RTS games has grown rapidly in the last few years, as
shown in \Cref{fig:rts-steam}.  This growth has been driven in part by
the democratization of game publishing, as embodied in game
distribution platforms such as Steam~\cite{steam}.  Censorship
circumventors can use this large body of games to avoid a censor's
attempt to block any particular game.

Further, since games within a given genre have common properties (\eg player 
moves and abstractions), any encoding scheme designed for one game is easily 
adaptable to another game within the same genre. These properties are listed
in Section \ref{subsec:rts}.



%% Further,
%% security features of games and their ability to leverage either a central
%% server or peer-to-peer architecture significantly raise the bar for censors. 

Finally, games may operate in two
architectural modes: (1) server-based where users connect to a server hosting
the games or (2) peer-to-peer where players connect directly to each other. The
first mode is advantageous, as clients using the covert channel look just like
any other game client connecting to the server, from the point of view of the
censor. However, the game server presents an easy target for blocking if the
censor is willing to incur the collateral damage. The second mode mitigates
this issue, but has weaker deniability if the censor is able to learn the IPs of
players acting as proxies for the covert traffic. Having both of these options
allows the covert channel to operate in whatever mode is most common in the
game and then switch to the alternate mode if the primary one is blocked.


Finally, 
%as we will demonstrate with our prototype ( \systemname), 
game-based 
covert channels can be designed such that they match the three properties 
highlighted by Geddes \etal while remaining resilient to censors that exploy
IP and port filtering, deep-packet inspection, flow-level traffic 
fingerprinting, active traffic manipulation, and even application-layer
attacks.

The idea of using video games for covert communication is not entirely
new.  Zander \etal\cite{Zander-1, Zander-2} were the first to propose
using first-person shooter video games for building covert channels
and the idea was recently revisited by Vines and Kohno
\cite{rook}However, \systemname (which is
the first covert channel to work over \rts games) offers several
crucial advantages over these systems.

\begin{packeditemize} 
\item {\bf Performance:} \systemname in its current implementation with a 
game-specific configuration achieves throuput rates that are over 200 times
higher than the work of Zander \etal \cite{Zander-1, Zander-2} and close to
106 times higher than Rook \cite{rook}. This makes \systemname
significantly more usable for establishing interactive covert communication 
channels.

\item {\bf Extensibility:} With only a few hours of coding effort, \systemname can
turn existing \rts games into covert channels. Unlike other game based covert
channels, \systemname
requires no understanding of how game commands and actions are coded into
network packets. \systemname only requires knowledge of how to decode game
replay files. For many games, tools to decode files are made readily available 
%which do this have already been made 
%available
by the gaming and hacking communities (for example, on many gaming
forums \cite{hacking-forum, hacking-forum-1, hacking-forum-2}).

\item {\bf Architectural Mobility:} While first-person-shooter games always operate
in client-server mode, \rts games often permit both -- client/server games and
\emph{direct connect} (peer-to-peer) games. As a consequence, for covert channels 
using first-person shooters, the game server is an easy target for blocking. In contrast, an \rts game-based 
covert channel can easily switch to peer-to-peer mode to evade blocking of the server.
%the face of this 
%threat, \rts games often present the advantage of mobility to a peer-to-peer 
%mode. 
\end{packeditemize}



%\iffalse In this paper, we argue that online games have multiple features that
%make them an ideal vector for covert communication. Further, as we evaluate our
%prototype, we investigate its ability to match the three properties highlighted
%by Geddes\etal and find that video game covert channels are able to match
%architectural, reliability and content properties of existing games. 
%
%revisit the idea of covert communication using video games as a covert channel.
%We find that the class of video games we consider, real-time strategy games,
%are amendable to cover communications and avoid the three mismatches outlined
%above. 
%
%\FIXME{Censorship arms race. Circumvention tools that try to look like other
%things.  Parrot is dead, cover your acks. This is the first (??) paper to use
%the cover your acks principles to design a circumvention system (not the
%fanciest claim ..  but maybe something we can claim? first people to take those
%principles and implement them in practice). } \fi
%


==> propertiesofcovert.tex <==
subsection{Properties of a good covert channel medium}

\Pnote{My feeling is these may come out in some sort of discussion section later on .. this feels a bit meta and we don't actually meet most of them.}


A covert channel embeds information in another channel, which we call
the {\textit medium} of the covert channel.  For example, the Freewave
covert channel uses Skype voice communications as its underlyng
medium.

A good covert channel for internet censorship circumvention must have
two key features: (1) it must provide good bandwidth and (2) it must
not be easy for an adversary to block.  These requirements impose
several constraints on the underlying medium for the channel.

\paragraph*{Good bandwidth.}  The channel cannot provide more bandwidth 
than the underlying medium, so the medium must also have good
bandwidth.

\paragraph*{Plausible deniability.}  The medium must have a 
``legitimate'' use.

\paragraph*{Economically valuable.}  The censor must have an incentive 
not to block the medium entirely.  For example, a censor is less
likely to block a medium that has a legitimate use that is
economically or socially valuable.

\paragraph*{Content-insensitive.}  Observable features of the medium, 
such as packet size, direction, and frequency, must be insensitive to
the content being carried by the medium.  Otherwise an adversary might
be able to detect when the medium is being used for censorship
circumvention and block those uses.  Among other things, this implies
that the medium should encrypt its data even when not used for
censorship circumvention.

\paragraph*{Authentication and access control.}  

\paragraph*{Oblivious intermediaries.}

\paragraph*{Diverse and rapidly adaptable.}

\paragraph*{International.}

